Maximum A Posteriori Direction-of-Arrival Estimation via Mixed-Integer Semidefinite Programming

We propose a joint sparse maximum a posteriori (MAP) estimator for DOA estimation from multiple snapshots, reformulated as a mixed-integer semidefinite program (MISDP). This enables efficient computation of globally optimal solutions using off-the-shelf MISDP solvers based on the branch-and-bound method. Unlike other nonconvex approaches for joint sparse recovery, such as the greedy methods and sparse Bayesian learning techniques, it provides a solution with an optimality assessment even with early termination. Additionally, we present a more scalable approximate solution approach for the MISDP problem based on randomized rounding. Numerical simulations demonstrate the improved threshold behavior, resolution, and robustness of our proposed method against popular DOA estimation methods. In particular, the proposed method applied with the randomized rounding algorithm exhibits a superior estimation performance at a significantly reduced running time, compared to the deterministic maximum likelihood (DML) estimator.

==> figures/tikzMacros.tex <==
% reduce linespacing in  legends
\pgfplotsset{every axis legend/.append style={row sep=-3pt, inner ysep=0pt, inner xsep=2pt}}


% % for colorbars
% \pgfplotsset{colorbar/draw/.code={
%       \begin{axis}[
%         colormap/jet,
%         colorbar horizontal,
%         every colorbar,
% 		at={(0.5,1.1)},
% 		anchor=south,
% 		height=5pt,
% 		xticklabel pos=upper,
%         colorbar shift,
%         colorbar=false,
%       ]
%         \pgfkeysvalueof{/pgfplots/colorbar addplot}
%       \end{axis}
%     }]
% }

% alignment of tikzpictures in text
\tikzset{every picture/.append style={baseline=(current bounding box.north west)}}

%\colorlet{cs1}{black!60!green}
%\colorlet{cs2}{black!25!orange}
%\colorlet{cs3}{blue!70!red}

% some parameters for the model images
%\colorlet{cs0}{black!50!gray}
%\colorlet{cs1}{black!60!green}
%\colorlet{cs2}{black!25!orange}
%\colorlet{cs3}{blue!70!red}
\colorlet{cs0}{black!30!yellow}
\colorlet{cs1}{black!30!red}
\colorlet{cs2}{white!30!blue}
\colorlet{cs3}{black!25!green}
\colorlet{cs4}{black!25!yellow}


\tikzstyle{sensor}=[anchor=center,circle, fill=cs0, inner sep=0pt, minimum height=1.5mm]
\tikzstyle{source}=[anchor=center,fill=red, inner sep=0pt, minimum height=1.5mm, minimum width=1.5mm]

%\tikzstyle{sensor}=[circle, fill=cs0, inner sep=0pt, minimum height=1.5mm]
%\tikzstyle{source}=[fill=red, inner sep=0pt, minimum height=1.5mm, minimum width=1.5mm]
\tikzstyle{sensorBg}=[line width=3mm, line join=round, cap=round, fill=black!10, draw=black!10]
\tikzstyle{mybox} = [draw=blue!60, thick, rectangle, rounded corners, inner sep=10pt, inner ysep=15pt]
\tikzstyle{myboxsmall} = [draw=blue!60, thick, rectangle, rounded corners, inner sep=10pt, inner ysep=7.5pt]
\tikzstyle{fancytitle} =[fill=blue!60, text=white, rounded corners]

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground} 

\def\NSen{6}
\def\NSnp{4}
\def\NGrd{12}
\def\dA{3}
\def\dB{5}
\def\dC{10}
\def\seedA{107}
\def\seedB{198}
\def\cRange{60}
\def\bSizeMod{1.7mm}


% colormap for mtrix color random generator
\newcommand{\cla}{\pgfmathdeclarerandomlist{color}{{red}{red}{orange}};}
\newcommand{\clb}{\pgfmathdeclarerandomlist{color}{{green}{green}{lime}};}
\newcommand{\clc}{\pgfmathdeclarerandomlist{color}{{blue}{blue}{teal}};}
\newcommand{\cld}{\pgfmathdeclarerandomlist{color}{{brown!60!black}{brown}{gray}};}
\newcommand{\cle}{\pgfmathdeclarerandomlist{color}{{olive!60!black}{olive}{gray}};}

% seed for random number generator
\def\seedA{20}
\def\seedB{500}
\def\bs{4.5pt}

% number of grid points and number of time samples
\def\varN{16}
\def\varT{30}

\def\doaA{4}
\def\doaB{7}
\def\doaC{13}

% full matrix
\newcommand{\drawMtx}[4]{
	\begin{tikzpicture}
		#1
		\pgfmathsetseed{\seedA}
		\foreach \x in {1,...,#3}{
		\foreach \y in {1,...,#2}{
			\pgfmathrandomitem{\c}{color};
			\pgfmathrandominteger{\r}{75}{100};
			\fill[\c!\r] (\x*#4, \y*#4) rectangle +(#4,#4);
		}
		}
	\end{tikzpicture}
}

% full matrix
\newcommand{\drawMtxB}[4]{
	\begin{tikzpicture}
		\foreach \x in {1,...,#3}{
		\foreach \y in {1,...,#2}{			
			\pgfmathrandominteger{\r}{50}{100};
			\fill[#1!\r] (\x*#4, \y*#4) rectangle +(#4,#4);
		}
		}
	\end{tikzpicture}
}

\newcommand{\rowSparseMtx}{
  \begin{tikzpicture}
	  
	  \draw[step=\bs,lightgray!50,very thin] (0,0) grid (\varT*\bs,-\varN*\bs);
	  
	  \node[anchor=south west,inner sep=0,outer sep=0] at (0,-\doaA*\bs) {\drawMtx{\cla}{1}{\varT}};
	  \node[anchor=south west,inner sep=0,outer sep=0] at (0,-\doaB*\bs) {\drawMtx{\clb}{1}{\varT}};
	  \node[anchor=south west,inner sep=0,outer sep=0] at (0,-\doaC*\bs) {\drawMtx{\clc}{1}{\varT}};	  
		
	  \draw (0,0) rectangle (\varT*\bs,-\varN*\bs);
	  
	  \node[anchor=south] at (0.5*\varT*\bs,-\varN*\bs-4ex) {$\mb{X}$};
				
  \end{tikzpicture}
}

\newcommand{\coVarMtx}{
  \begin{tikzpicture}
	  
	  \draw[step=\bs,lightgray!50,very thin] (0,0) grid (\varN*\bs,-\varN*\bs);
	  
	  \foreach \x in {\doaA, \doaB, \doaC}{
	  \foreach \y in {\doaA, \doaB, \doaC}{
		  \pgfmathrandominteger{\r}{50}{100};
		  \fill[gray!\r] (\x*\bs-\bs, -\y*\bs+\bs) rectangle +(\bs,-\bs);
	  }
	  }
	  
	  \fill[red!80] (\doaA*\bs-\bs, -\doaA*\bs+\bs) rectangle +(\bs,-\bs);
	  \fill[green!100]  (\doaB*\bs-\bs, -\doaB*\bs+\bs) rectangle +(\bs,-\bs);
	  \fill[blue!100]   (\doaC*\bs-\bs, -\doaC*\bs+\bs) rectangle +(\bs,-\bs);
	  
	  \draw (0,0) rectangle (\varN*\bs,-\varN*\bs);
	  
	  \node[anchor=south] at (0.5*\varN*\bs,-\varN*\bs-4ex) {$\hat{\mb{P}} = \mb{X} \mb{X}^{H} $};
				
  \end{tikzpicture}
}

\newcommand{\sparseStruct}{
  \begin{tikzpicture}   
	\node[anchor=north east] (rs) at (-5mm,0) {\rowSparseMtx};
	\node[anchor=north] at (0,-0.5*\varN*\bs) {$\Rightarrow$};
	\node[anchor=north west] (cs) at (5mm,0) {\coVarMtx};
  \end{tikzpicture}
}

